Unraveling the Complexity of Dwarf Galaxy Dynamics: A study of Binary Orbital Motions

We investigate the impact of binary orbital motions on the dynamical modeling of dwarf galaxies with intrinsic line-of-sight velocity dispersions ($\sigma_{v_r}$) of 1 to 9 km/s. Using dwarf galaxies from the Auriga level-2 and level-3 simulations, we apply the Jeans Anisotropic Multi-Gaussian Expansion modelling to tracer stars before and after including binaries to recover the dynamical masses. The recovered total masses within the half-mass radius of tracers, $M(<r_\mathrm{half})$, are always inflated due to binary motions, with greater inflations occurring for smaller $\sigma_{v_r}$. However, many dwarf galaxies experience central density deflated due to binary motions, with little dependences on $\sigma_{v_r}$. This is due to the negative radial gradients in the velocity dispersion profiles, with the fractional inflation in $\sigma_{v_r}$ due to binaries more significant in outskirts. An extreme binary fraction of 70% can lead to central density deflation of up to 10-20% at 3 km/s$<\sigma_{v_r}<$8 km/s, with $M(<r_\mathrm{half})$ inflated by 4% at 9 km/s and up to 15% at 3 km/s. A lower binary fraction of 36% leads to similar deflations, with the inflations decreasing to approximately 10% at 3 km/s and becoming statistically insignificant. The choice of binary orbit distribution models does not result in significant differences, and observational errors tend to slightly weaken the deflations in the recovered central density. Two observations separated by one year to exclude binaries lead to almost zero inflations/deflations for a binary fraction of 36% over 3 km/s$<\sigma_{v_r}<$9 km/s. For $\sigma_{v_r}\sim$1 km/s to 3 km/s, a binary fraction of 70% (36%) still results in 60% (30%) to 10% (1%) of inflations in $M(<r_\mathrm{half})$, even with two-epoch observation.

==> Makefile <==
MAIN=paper
OLD=old/paper
BIB=master.bib
STYLE=mnras.cls mnras.bst
#timestr=`date +%a-%d-%b`
timestr=`date -Idate`
#lineno.sty
TC=pdflatex

ifeq ($(TC), latex)
PC=dvipdf
else
PC=echo
endif

paper:
	$(TC) $(MAIN)
	bibtex $(MAIN)
	$(TC) $(MAIN)
	$(TC) $(MAIN)
	$(PC) $(MAIN)

diff:
	latexdiff $(OLD).tex $(MAIN).tex >diff.tex
	@make paper -e MAIN=diff
	@make clean -e MAIN=diff
	
tar: clean paper 
	mkdir tmp
	mkdir tmp/figures
	cp $(MAIN).tex $(MAIN).bbl $(BIB) $(STYLE) Makefile tmp/
	cp figures/*.pdf tmp/figures/
	cd tmp;	tar -czhf $(MAIN).$(timestr).tar.gz *; mv $(MAIN).$(timestr).tar.gz ../
	
clean:
	\rm -rf tmp
	\rm -f $(MAIN).aux $(MAIN).log $(MAIN).toc $(MAIN).blg $(MAIN).dvi $(MAIN).ps $(MAIN).out $(MAIN).bbl
	\rm -f diff.aux diff.log diff.toc diff.blg diff.dvi diff.ps diff.out diff.bbl

ultclean:
	\rm -rf tmp
	\rm -f *.aux *.log *.toc *.blg *.dvi *.ps *.out *.bbl *.backup $(MAIN).*.tar.gz $(MAIN).pdf
	\rm -f diff.pdf diff.tex


